Learning Debiased and Disentangled Representations for Semantic Segmentation

Deep neural networks are susceptible to learn biased models with entangled feature representations, which may lead to subpar performances on various downstream tasks. This is particularly true for under-represented classes, where a lack of diversity in the data exacerbates the tendency. This limitation has been addressed mostly in classification tasks, but there is little study on additional challenges that may appear in more complex dense prediction problems including semantic segmentation. To this end, we propose a model-agnostic and stochastic training scheme for semantic segmentation, which facilitates the learning of debiased and disentangled representations. For each class, we first extract class-specific information from the highly entangled feature map. Then, information related to a randomly sampled class is suppressed by a feature selection process in the feature space. By randomly eliminating certain class information in each training iteration, we effectively reduce feature dependencies among classes, and the model is able to learn more debiased and disentangled feature representations. Models trained with our approach demonstrate strong results on multiple semantic segmentation benchmarks, with especially notable performance gains on under-represented classes.

==> sections/limitations.tex <==
\section{Limitations \& Negative Societal Impact}
\label{sec:limitations}

One limitation of the proposed DropClass training scheme is that it requires more iterations for the model to fully converge. 
This is because DropClass depends on the model's ability to generate disentangled feature representations. Hence, the model must be trained with ordinary supervision first, which is also the reason we ramp up $\lambda$ from 0 to 1 during training. 

The negative societal impact of our work do not necessarily pertain to our work itself, but moreso to deep learning and semantic segmentation. 
Semantic segmentation, and deep learning in general, requires massive amounts labeled data to train the model. 
As more and more large-scale datasets are created and made public, one natural point of concern is privacy. 
For example, even the datasets that we use --- Cityscapes and Pascal VOC --- both have images containing people; people who most likely are completely unaware that pictures of them are being used by machine learning researchers all over the world.
Although we do not know the extent of negative impact this would have on society, concerns over privacy is definitely something that needs to be considered when curating new datasets.

